TRIVEA: Transparent Ranking Interpretation using Visual Explanation of Black-Box Algorithmic Rankers

Ranking schemes drive many real-world decisions, like, where to study, whom to hire, what to buy, etc. Many of these decisions often come with high consequences. For example, a university can be deemed less prestigious if not featured in a top-k list, and consumers might not even explore products that do not get recommended to buyers. At the heart of most of these decisions are opaque ranking schemes, which dictate the ordering of data entities, but their internal logic is inaccessible or proprietary. Drawing inferences about the ranking differences is like a guessing game to the stakeholders, like, the rankees (i.e., the entities who are ranked, like product companies) and the decision-makers (i.e., who use the rankings, like buyers). In this paper, we aim to enable transparency in ranking interpretation by using algorithmic rankers that learn from available data and by enabling human reasoning about the learned ranking differences using explainable AI (XAI) methods. To realize this aim, we leverage the exploration-explanation paradigm of human-data interaction to let human stakeholders explore subsets and groupings of complex multi-attribute ranking data using visual explanations of model fit and attribute influence on rankings. We realize this explanation paradigm for transparent ranking interpretation in TRIVEA, a visual analytic system that is fueled by: i) visualizations of model fit derived from algorithmic rankers that learn the associations between attributes and rankings from available data and ii) visual explanations derived from XAI methods that help abstract important patterns, like, the relative influence of attributes in different ranking ranges. Using TRIVEA, end users not trained in data science have the agency to transparently reason about the global and local behavior of the rankings without the need to open black-box ranking models and develop confidence in the resulting attribute-based inferences. We demonstrate the efficacy of TRIVEA using multiple usage scenarios and subjective feedback from researchers with diverse domain expertise. Keywords: Visual Analytics, Learning-to-Rank, Explainable ML, Ranking

==> sections/conclusion.tex <==
\section{Conclusion}
%TODO

==> sections/discussion.tex <==
\section{Discussion}
%TODO

==> sections/introduction.tex <==
\firstsection{Introduction}

\maketitle


Rankings are convenient heuristics for the human mind to make quick decisions. Which food to buy, which product to order, or which educational institutions to attend -– in many cases, ordering of data entities, like restaurants, products, and universities, come with high socio-technical consequences. For example, a university that is not in the top-k list can be deemed as less prestigious or a product that is not recommended to buyers can lose substantial amounts in revenue. The ordering i

%Rankings serve as an efficient decision heuristic for making selections among a set of alternatives. The underlying complexity of the data space is often hidden from the consumer. For example, a search interface for universities can help students generate customized rankings based on their preferences for school selection. However, students may be interested in what makes the top-$10$ schools different from schools ranked $40$ to $50$, so they can make decisions on what schools to apply. Additionally, we can also imagine the university administrators wish to gain knowledge about the key rank stimulators in higher or lower rank ranges in reference to their competitor schools, so they can decide on strategies of improving their rankings.

\aritra{We build a visual analytic workflow that is fueled by supervised learning algorithms}
The latter scenario can be addressed by learning from data using past rankings. We assume the signals of ranking stimulators remains in the feature and ranking data.
The former scenario can also benefit from not only comparing the school differences regard to feature values but also the importance of the feature to the rankings.

Modeling is a means to an end of discovering those signals  but those signals need to be accessed and communicated to humans. We preserve human agency~\cite{heer2019agency,shneiderman2021human} by visualization as a transparent means to access model outputs and their explanations. 
Different from a search engine that require users to provide the ranking  formulas, we argue that there is less burden on the information consumer (i.e., a student to university ranking) to alter the ranking formulas by indicating their preferences of models which preserves the associations among rankings and features. Besides information consumers, inferences directly from modeling the history ranking are also essential for the ranked entities, like universities or businesses to catch up with their peers. For example, the formula for generating university ranking are vague, opaque, or not applicable for certain ranking ranges. Hence, the models learned on the data may expose more complicated decision rules associate to the schools and their nearby peers. 


The focus of our work is on developing algorthmic rankers, where learning-to-rank~(LTR) algorithms are applied to historical ranking data, resulting in models that learn a scoring function from labeled data. A scoring function is a substitute of the actual ranking formula. 
The learned scoring function is difficult to express in a concise mathematical formula as local data neighborhoods have a high degree of variance..\aritra{reword} 
However, the problem with LTR models is that summary performance metrics may not capture their performance  in local data neighborhoods, let alone the local model behaviors.
We define the local model behaviors as the association of features and ranking locally, which is an essential information for people who want to make informed judgments based on these rankings. 
However, the local ranking behavior can vary even if the ranking is generated from the same close form scoring function [citation of Julia’s paper], let along the complex scoring function learned by models.


For aiding in such data-driven inference tasks, we develop \texttt{RIEVAL}, for ranking explanation and evaluation using visual analysis of LTR models. \texttt{RIEVAL} leverages multi-model comparison of ranking performance and explanations and thereby addresses the need for facilitating comparative analysis in post-hoc model interpretation tasks~\cite{hong2020human} .

As part of the development of \texttt{RIEVAL}, we have three key contributions in this paper:
i) conceptualize how reasoning can be facilitated by leveraging visual analytics with appropriate adaption of LTR models and LIME model explanation method~(Figure~\ref{figs:overview}),
ii) design and development of an interactive interface for post-hoc analysis across models, explanations, and time for model evaluation and reasoning.
iii) demonstration the efficacy of \texttt{RIEVAL} in solving real-world data analysis tasks involving ranked entities, through multiple usage scenarios and subjective feedback from data science experts.
%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sections/method.tex <==

\section{Methodology}
\label{sec:method}
In this section, we describe the methodology used for data abstraction, model training, model explaining. We performed those steps and imported the data into our interface post-hoc.



\textbf{Data pre-processing} For learning from historical data, for example, the university ranking dataset ~\cite{University} does not naturally include the element of query-document pair and label defined in the information retrieval context. In information retrieval, query-document pair is a search keyword to a webpage, and the relevant score is measuring how related the webpage is to the keyword~\cite{salton2003information}. If we have the university ranking from the last ten years, year value is the unique identifier of a ranking list. Hence, it is reasonable to use the year as the query id. We can imagine a search keyword “2021”. It returns the list of universities ordered by their ranking from the top to the bottom, in year 2021. In this scenario, the query is the year; a document is analogous to the school represented by its features; the label is the ranking of the school. In summary, to apply the LTR methods to any data set, one would need to first identify the label, query, and document in the data.



\textbf{Model training} 
Various methods have been developed to model ranking data. In general, they can be categorized to white-box methods and black-box methods. white-box methods include the traditional mathematical methods such as Analytic Hierarchy Process models~\cite{dyer1990remarks} (with Saaty’s and Koczkodaj’s inconsistencies~\cite{bozoki2008saaty}), probability models (Luce model~\cite{cheng2010label}, distance-based model~\cite{fligner1986distance}, and rank-ordered logit model~\cite{fok2012rank}). The black-box methods include the Machine Learning and Deep Learning methods that are widely explored in the web page rankings for Information Retrieval purposes,. We chose LTR models since it is effective in IR ranking scenarios but not been explored enough on other ranking tasks. And we assume that LTR methods have the potential for handling complicated ranking data than the traditional mathematical methods.
We used the Ranklib toolkit\cite{RankLib} from the Lemur Project for model training. The input data was converted during the data abstraction to the format used in LETOR datasets in order to be compatible for the algorithms. Then, we selected several pointwise, pairwise, and listwise LTR algorithms in our training phase. During the experimentation phase, we used different training metrics for the listwise algorithms to see if the training metrics impact the model performance. We used  \textit{MAP}, \textit{NDCG@10}, and \textit{NDCG@50}. However, we observed that the AdaRank algorithm trains unsuccessfully across all three datasets. For Coordinate Ascent and LambdaMART, using \textit{NDCG@10} or \textit{NDCG@50} does not make a significant difference.  Hence in this work, we use \textit{NDCG@10}, a commonly used metric in the information retrieval context, as the training metric, if the algorithm requires a training metric. 


\textbf{Model explaining} Explanations are required to connect rankings with the features responsible for high or low ranks, as detected by a LTR model. It is a common practice for a non-expert to treat machine learning models as black boxes and abstract the explanation by investigating the input-output pairs. A widely adopted model-agnostic explanation technique is LIME (Locally Interpretable Model Explanations)
\cite{ribeiro2016modelagnostic}. 
LIME is widely used in explaining machine learning models in classification~(i.e., in image recognition and natural language processing tasks). 
It explains the model output result of a single item but differs from the global explanation method since the local explanation tends to be simpler and more accurate. LIME generates samples for each data item based on the feature space, feeding those simulated samples to the model to obtain the outputs to those samples. 
Then a local linear regression is performed on the input output pairs of sample data, which generates the weights of the features in the local scope. 
Those feature weights values can be positive or negative, impacting the specific item locally. 
A  traditional global explanation , which summarize the feature importance for an entire data set , cannot provide sufficient insight on the decision-making process of models in the local neighborhoods, which is the focus of our work.
LIME technique overcomes the limitations of global explanations and is useful when the underlying relationship between the features and the outcomes is simple. 
The LIME method explains that for a single item, how much each  feature contributes to the output. The explanation of a classification task is the percentage of instances that belong to a certain class along with its support and resistance factors.
But for ranking, which is an ordinal variable, we have much more unique values than the number of classes in a classification task. For ranking tasks, the explanation is the rank position, and factors stimulate its improvement. And the stimulation on ranking will only be triggered when the positive effect from a feature is significant enough to change the output ranking. Hence, the LIME explanation results for the LTR model indicate the feature contributions to move the instance up at least one rank.

Although there are other explanation methods, such as SHAP, we prefer the LIME method to aid the reasoning of the ranking model output. The explanation from SHAP is a contrastive explanation that compares the model output to the average model output. In  a binary 0-1 classification case, the average model output is the average probability score for an item belonging to class 1. But the average probability for an item getting a rank promotion is hard to interpret, since if all rank items get a promotion, the rank will stay the same. 
After the models were trained, we used the LIME package\cite{LimeRepo} in Python to generate samples from input features, convert the samples to LETOR format, and then generate explanations from all input data points.


















==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


